NLO QCD and electroweak corrections to $Z+\gamma$ production with leptonic Z-boson decays

The next-to-leading-order electroweak corrections to $pp\to l^+l^-/\bar\nu\nu+\gamma+X$ production, including all off-shell effects of intermediate Z bosons in the complex-mass scheme, are calculated for LHC energies, revealing the typically expected large corrections of tens of percent in the TeV range. Contributions from quark-photon and photon-photon initial states are taken into account as well, but their impact is found to be moderate or small. Moreover, the known next-to-leading-order QCD corrections are reproduced. In order to separate hard photons from jets, both a quark-to-photon fragmentation function \'a la Glover/Morgan and Frixione's cone isolation are employed. The calculation is available in the form of Monte Carlo programs allowing for the evaluation of arbitrary differential cross sections. Predictions for integrated cross sections are presented for the LHC at 7 TeV, 8 TeV, and 14 TeV, and differential distributions are discussed at 14 TeV for bare muons and dressed leptons. Finally, we consider the impact of anomalous $ZZ\gamma$ and $Z\gamma\gamma$ couplings.

==> plots/feynman_diagrams/setup.tex <==
\renewcommand{\topfraction}{0.7}
\renewcommand{\bottomfraction}{1.0}
\renewcommand{\textfraction}{0.3}
\renewcommand{\floatpagefraction}{0.7}

% new commands for cross referencing
\def\refeq#1{\mbox{(\ref{#1})}}
\def\reffi#1{\mbox{Fig.~\ref{#1}}}
\def\reffis#1{\mbox{Figs.~\ref{#1}}}
\def\refta#1{\mbox{Table~\ref{#1}}}
\def\reftas#1{\mbox{Tables~\ref{#1}}}
\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refses#1{\mbox{Sections~\ref{#1}}}
\def\refapp#1{\mbox{App.~\ref{#1}}}
\def\refapps#1{\mbox{Apps.~\ref{#1}}}
\def\citere#1{\mbox{Ref.~\cite{#1}}}
\def\citeres#1{\mbox{Refs.~\cite{#1}}}

% shorthands for greek letters
\def\al{\alpha}
\def\be{\beta}
\def\ga{\gamma}
\def\de{\delta}
\def\veps{\varepsilon}
\def\la{\lambda}
\def\si{\sigma}
\def\Ga{\Gamma}
\def\De{\Delta}
\def\La{\Lambda}

% physical units (math-mode is removed)
% -> direct use in math-environment is possible
\newcommand{\eV}{\unskip\,\mathrm{eV}}
\newcommand{\GeV}{\unskip\,\mathrm{GeV}}
\newcommand{\MeV}{\unskip\,\mathrm{MeV}}
\newcommand{\TeV}{\unskip\,\mathrm{TeV}}
\newcommand{\fba}{\unskip\,\mathrm{fb}}
\newcommand{\mba}{\unskip\,\mathrm{mb}}
\newcommand{\pba}{\unskip\,\mathrm{pb}}
\newcommand{\nba}{\unskip\,\mathrm{nb}}

%physical particles
\def\mathswitch#1{\relax\ifmmode#1\else$#1$\fi}
\def\mathswitchr#1{\relax\ifmmode{\mathrm{#1}}\else$\mathrm{#1}$\fi}
\def\mathswitchit#1{\relax\ifmmode{#1}\else$#1$\fi}

% generic fields
\newcommand{\PHgeneric}{\mathswitchr \phi^0}
\newcommand{\Pf}{f}
\newcommand{\Ph}{\mathswitchr h}
\newcommand{\Pj}{\mathswitchr j}
% proton and quarks
\newcommand{\Pu}{u}
\newcommand{\Pd}{d}
\newcommand{\Ps}{s}
\newcommand{\Pc}{c}
\newcommand{\Pt}{\mathswitchr t}
\newcommand{\Pp}{\mathswitchr p}
\newcommand{\Ppbar}{\overline{\Pp}}
\newcommand{\Pq}{\mathswitchit q}
% charged leptons
\newcommand{\Pl}{\mathswitch l}
\newcommand{\Plp}{\mathswitch l^+}
\newcommand{\Plm}{\mathswitch l^-}
\newcommand{\Pe}{\mathswitchr e}
\newcommand{\Pep}{\mathswitchr {e^+}}
\newcommand{\Pem}{\mathswitchr {e^-}}
\newcommand{\Pepm}{\mathswitchr {e^\pm}}
\newcommand{\Pmu}{\mathswitchr {\mu}}
\newcommand{\Pmum}{\mathswitchr {\mu^-}}
% gauge bosons
\newcommand{\PWp}{\mathswitchr {W^+}}
\newcommand{\PWm}{\mathswitchr {W^-}}
\newcommand{\PWpm}{\mathswitchr {W^\pm}}
\newcommand{\PWO}{\mathswitchr {W^0}}
\newcommand{\PZO}{\mathswitchr {Z^0}}
\newcommand{\PB}{\mathswitchr B}
\newcommand{\PW}{\mathswitchr W}
\newcommand{\PZ}{\mathswitchr Z}
\newcommand{\PAn}{\mathswitchr {A^0}}
\newcommand{\Pg}{g}
\newcommand{\PH}{\mathswitchr H}
% Higgs-fields
\newcommand{\PHu}{\mathswitchr H_\Pu}
\newcommand{\PHd}{\mathswitchr H_\Pd}
\newcommand{\Phn}{\mathswitchr {h^0}}
\newcommand{\PHn}{\mathswitchr {H^0}}
% neutrinos
\newcommand{\Pnl}{\mathswitch {\nu_\Pl}}
\newcommand{\Pne}{\mathswitch \nu_{\mathrm{e}}}
\newcommand{\Panl}{\mathswitch {\bar\nu_\Pl}}
\newcommand{\Pane}{\mathswitch \bar\nu_{\mathrm{e}}}
\newcommand{\Pnmu}{\mathswitch \nu_\mu}

% particle masses
\newcommand{\MB}{\mathswitch {M_\PB}}
\newcommand{\Mf}{\mathswitch {m_\Pf}}
\newcommand{\Ml}{\mathswitch {m_\Pl}}
\newcommand{\Mq}{\mathswitch {m_\Pq}}
\newcommand{\MV}{\mathswitch {M_\PV}}
\newcommand{\MW}{\mathswitch {M_\PW}}
\newcommand{\hMW}{\mathswitch {\hat M_\PW}}
\newcommand{\MWpm}{\mathswitch {M_\PWpm}}
\newcommand{\MWO}{\mathswitch {M_\PWO}}
\newcommand{\MA}{\mathswitch {M_\PAn}}
\newcommand{\MZ}{\mathswitch {M_\PZ}}
\newcommand{\MH}{\mathswitch {M_\PH}}
\newcommand{\Me}{\mathswitch {m_\Pe}}
\newcommand{\Mmy}{\mathswitch {m_\mu}}
\newcommand{\Mta}{\mathswitch {m_\tau}}
\newcommand{\Md}{\mathswitch {m_\Pd}}
\newcommand{\Mu}{\mathswitch {m_\Pu}}
\newcommand{\Ms}{\mathswitch {m_\Ps}}
\newcommand{\Mc}{\mathswitch {m_\Pc}}
\newcommand{\Mb}{\mathswitch {m_\Pb}}
\newcommand{\Mt}{\mathswitch {m_\Pt}}
\newcommand{\GW}{\mathswitch {\Gamma_\PW}}
\newcommand{\GZ}{\mathswitch {\Gamma_\PZ}}

\newcommand{\Mhn}{\mathswitch {M_{\Phn}}}
\newcommand{\MHn}{\mathswitch {M_{\PHn}}}
\newcommand{\MHgeneric}{\mathswitch {M_{\PHgeneric}}}
\newcommand{\Mhntree}{\mathswitch {m_{\Phn}}}
\newcommand{\MHntree}{\mathswitch {m_{\PHn}}}

% complex masses
\newcommand{\muw}{\mathswitch {\mu_{\PW}}}

% shorthands for SM parameters
\newcommand{\scrs}{\scriptscriptstyle}
\newcommand{\sw}{\mathswitch {s_{\scrs\PW}}}
\newcommand{\cw}{\mathswitch {c_{\scrs\PW}}}

\newcommand{\swbar}{\mathswitch {\bar s_{\scrs\PW}}}
\newcommand{\swfbar}{\mathswitch {\bar s_{\PW,\Pf}}}
\newcommand{\swqbar}{\mathswitch {\bar s_{\PW,\Pq}}}
\newcommand{\Qf}{\mathswitch {Q_\Pf}}
\newcommand{\Ql}{\mathswitch {Q_\Pl}}
\newcommand{\Qq}{\mathswitch {Q_\Pq}}
\newcommand{\vf}{\mathswitch {v_\Pf}}
\newcommand{\af}{\mathswitch {a_\Pf}}
\newcommand{\gesi}{\mathswitch {g_\Pe}^{\sigma}}
\newcommand{\gem}{\mathswitch {g_\Pe}^-}
\newcommand{\gep}{\mathswitch {g_\Pe}^+}
\newcommand{\GF}{\mathswitch {G_\mu}}
\newcommand{\Qu}{\mathswitch {Q_u}}

\newcommand{\vev}{\mathswitch v}
\newcommand{\vevu}{\mathswitch v_\Pu}
\newcommand{\vevd}{\mathswitch v_\Pd}

\newcommand{\sina}{s_\alpha}
\newcommand{\cosa}{c_\alpha}
\newcommand{\sinb}{s_\beta}
\newcommand{\cosb}{c_\beta}
\newcommand{\tana}{t_\alpha}
\newcommand{\tanb}{t_\beta}
\newcommand{\cotb}{\cot \beta}

\hyphenation{brems-strah-lung}

%various shorthands
\def\ie{i.e.\ }
\def\eg{e.g.\ }
\def\cf{cf.\ }

% slashed quantities
\newcommand{\as}{a\hspace{-0.5em}/\hspace{0.1em}}
\newcommand{\es}{\varepsilon \hspace{-0.5em}/\hspace{0.1em}}
\newcommand{\ks}{k\hspace{-0.52em}/\hspace{0.1em}}
\newcommand{\ps}{p\hspace{-0.42em}/}%\hspace{0.1em}}
\newcommand{\qs}{q\hspace{-0.5em}/\hspace{0.1em}}
\newcommand{\hb}{h\hspace{-0.5em}\vspace{-0.3em}-\hspace{0.1em}}
\marginparwidth 1.2cm

% orders of magnitude
\newcommand{\ord}{{\cal O}}
\renewcommand{\O}{{\cal O}}
\newcommand{\Oa}{\mathswitch{{\cal{O}}(\alpha)}}

% various abbreviations
\newcommand{\rE}{{\mathrm{E}}}
\newcommand{\ri}{{\mathrm{i}}}
\newcommand{\re}{{\mathrm{e}}}
\newcommand{\rT}{{\mathrm{T}}}
\newcommand{\rM}{{\mathrm{M}}}
\newcommand{\ieps}{\ri\epsilon}
\newcommand{\rd}{{\mathrm{d}}}
\newcommand{\br}{{\mathrm{br}}}
\newcommand{\soft}{{\mathrm{soft}}}
\newcommand{\onel}{{\mathrm{1-loop}}}
\newcommand{\M}{{\cal {M}}}
\renewcommand{\L}{{\cal L}}
\newcommand{\F}{{\cal {F}}}
\newcommand{\bq}{{\bf q}}
\newcommand{\ehel}{\kappa}
\newcommand{\da}{\Delta\alpha}
\newcommand{\dr}{\Delta\rho}
\newcommand{\dLL}{\Delta_{\mathrm{LL}}}

\newcommand{\cut}{{\mathrm{cut}}}
\newcommand{\jet}{{\mathrm{jet}}}
\newcommand{\llog}{{\mathrm{LL}}}
\newcommand{\FSR}{{\mathrm{FSR}}}
\newcommand{\EW}{{\mathrm{EW}}}
\newcommand{\QCD}{{\mathrm{QCD}}}
\newcommand{\QED}{{\mathrm{QED}}}
\newcommand{\LEP}{{\mathrm{LEP}}}
\newcommand{\OS}{{\mathrm{OS}}}
\newcommand{\SLD}{{\mathrm{SLD}}}
\newcommand{\SM}{{\mathrm{SM}}}
\newcommand{\MSSM}{{\mathrm{MSSM}}}
\newcommand{\SUSY}{{\mathrm{SUSY}}}
\newcommand{\CM}{{\mathrm{CM}}}
\newcommand{\born}{{\mathrm{Born}}}
\newcommand{\virt}{{\mathrm{virt}}}
\newcommand{\coll}{{\mathrm{coll}}}
\newcommand{\sub}{{\mathrm{sub}}}
\newcommand{\ini}{{\mathrm{ini}}}
\newcommand{\fin}{{\mathrm{fin}}}
\newcommand{\fact}{{\mathrm{fact}}}
\newcommand{\nonfact}{{\mathrm{nonfact}}}
\newcommand{\res}{{\mathrm{res}}}
\newcommand{\rec}{{\mathrm{rec}}}
\newcommand{\PA}{{\mathrm{PA}}}
\newcommand{\real}{{\mathrm{real}}}
\newcommand{\veto}{{\mathrm{veto}}}
\newcommand{\LO}{{\mathrm{LO}}}
\newcommand{\NLO}{{\mathrm{NLO}}}
\newcommand{\Int}{{\mathrm{IF}}}

%various abbreviations by Markus

\newcommand{\SP}[1]{\langle#1\rangle}
\newcommand{\CSP}[1]{\langle#1\rangle^{\ast}}
\newcommand{\DSP}[3]{\langle#1|#2|#3\rangle}
\newcommand{\vkv}[4]{\left(\begin{array}{cc}#1&#2\\#3&#4\\\end{array}\right)}
\newcommand{\zv}[2]{\left(#1\,,#2\right)}
\newcommand{\sv}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)}
\newcommand{\pu}{p_{u}}
\newcommand{\pd}{p_{d}}
\newcommand{\pos}{l^{+}}
\newcommand{\kl}{k_{l}}
\newcommand{\kn}{k_{\nu}}
\newcommand{\kp}{k_{\gamma}}
\newcommand{\kg}{k_{g}}

\newcommand{\klnp}{k_{123}}
\newcommand{\slnp}{\hat{s}_{123}}

\newcommand{\qw}{q_{W}}
\newcommand{\muW}{\mu_{W}}
\newcommand{\alphas}{\alpha_{s}}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\intd}{\mathrm{d}}
\newcommand{\klam}[1]{\left(#1\right)}
\newcommand{\sh}{\hat{s}}
\newcommand{\md}{\mathrm{d}}
\newcommand{\mr}[1]{\mathrm{#1}}
\newcommand{\MtW}{M_{\mathrm{T},\Plp\nu}}
\newcommand{\MtWA}{M_{\mathrm{T},\Plp\nu\gamma}}


% mathematical functions
\def\atn{\mathop{\mathrm{arctan}}\nolimits}
\def\Li{\mathop{\mathrm{Li}_2}\nolimits}
\def\cLi{\mathop{{\cal L}i_2}\nolimits}
\def\Re{\mathop{\mathrm{Re}}\nolimits}
\def\Im{\mathop{\mathrm{Im}}\nolimits}
\def\sgn{\mathop{\mathrm{sgn}}\nolimits}
\def\arc{\mathop{\mathrm{arc}}\nolimits}

% Momenta
\newcommand{\pina}{\mathswitch {p_1}}
\newcommand{\Pina}{\mathswitch {p_1}}
\newcommand{\pinb}{\mathswitch {p_2}}
\newcommand{\Pinb}{\mathswitch {p_2}}
\newcommand{\knu}{\mathswitch {k_{\nu}}}
\newcommand{\Knu}{\mathswitch {k_{\nu}}}
\newcommand{\klb}{\mathswitch {k_{\Pl}}}
\newcommand{\Klb}{\mathswitch {k_{\Pl}}}
\newcommand{\kj}{\mathswitch {p_3}}
\newcommand{\Kj}{\mathswitch {p_3}}
\newcommand{\kga}{\mathswitch {k_{\ga}}}
\newcommand{\Kga}{\mathswitch {k_{\ga}}}
\newcommand{\kw}{\mathswitch {k_{\PW}}}
\newcommand{\Kw}{\mathswitch {k_{\nu}+k_{\Pl}}}

% Helicities
\newcommand{\siga}{\mathswitch {\sigma_1}}
\newcommand{\sigb}{\mathswitch {\sigma_2}}
\newcommand{\taulb}{\mathswitch {\tau_{\Pl}}}
\newcommand{\laj}{\mathswitch {\sigma_3}}
\newcommand{\laga}{\mathswitch {\lambda_{\ga}}}

% Processes
\newcommand{\udnlg}{\mathswitch {\Pu\bar{\Pd}\to\Pl^+\Pnl \mathrm{g}}}
\newcommand{\UDGG} {\mathswitch {\mathrm{gg}\Pd\Pu}}


\newcommand{\Pbbar}{{\bar{\Pb}}}
\newcommand{\Pdbar}{{\bar{\Pd}}}
\newcommand{\Pubar}{{\bar{\Pu}}}
\newcommand{\Pqbar}{{\bar{\Pq}}}
\newcommand{\MSbar}{{$\overline{\mathrm{MS}}$}}
\newcommand{\DRbar}{{$\overline{\mathrm{DR}}$}}

\newcommand{\phz}{\phantom{(0)}}

